Comparing Template-based and Template-free Language Model Probing

The differences between cloze-task language model (LM) probing with 1) expert-made templates and 2) naturally-occurring text have often been overlooked. Here, we evaluate 16 different LMs on 10 probing English datasets -- 4 template-based and 6 template-free -- in general and biomedical domains to answer the following research questions: (RQ1) Do model rankings differ between the two approaches? (RQ2) Do models' absolute scores differ between the two approaches? (RQ3) Do the answers to RQ1 and RQ2 differ between general and domain-specific models? Our findings are: 1) Template-free and template-based approaches often rank models differently, except for the top domain-specific models. 2) Scores decrease by up to 42% Acc@1 when comparing parallel template-free and template-based prompts. 3) Perplexity is negatively correlated with accuracy in the template-free approach, but, counter-intuitively, they are positively correlated for template-based probing. 4) Models tend to predict the same answers frequently across prompts for template-based probing, which is less common when employing template-free techniques.

==> newTable1.tex <==
\setlength{\tabcolsep}{2pt}
\centering\small\setlength{\tabcolsep}{6pt}
\begin{tabular}{llllll}
   \toprule
      \textbf{Template-based Probing} & \textbf{Template-free Probing} \\
    \midrule
        Template: “[X] born [MASK]” &  Template: N/A
 \\
 \midrule
        Peter F. Martin born [MASK]
 & \begin{tabular}[l]{@{}l@{}}Peter F Martin (born [MASK]) \\ is an American politician [...]\end{tabular}
 
 % &  Peter F Martin (born [MASK]) is an American politician [...]
 \\
        Dennis B. Sullivan born [MASK]

 % &  Sullivan was born in Chippewa Falls, Wisconsin in [MASK]
 & \begin{tabular}[c]{@{}c@{}}Sullivan was born in Chippewa Falls \\ Wisconsin in [MASK]\end{tabular} 
 \\
        Tan Jiexi born [MASK]

  & \begin{tabular}[c]{@{}c@{}}Tan Jiexi (born December 2, [MASK] in \\ Shenzhen,China), is a Chinese singer-songwriter\end{tabular} 

 % &  Tan Jiexi (born December 2, [MASK] in Shenzhen,China), is a Chinese singer-songwriter
 \\
        Tasos Neroutsos born [MASK]


   & \begin{tabular}[l]{@{}c@{}}Neroutsos was born in Athens in \\ [MASK] to a wealthy family\end{tabular} 

 % &  Neroutsos was born in Athens in [MASK] to a wealthy family

 \\

     \bottomrule
  \end{tabular}
% \caption{Template-based and template-free probing examples from the LAMA: Google-RE dataset.} 
\label{main_figure}
